A User-centered Approach for Optimizing Information Visualizations

The optimization of information visualizations is time consuming and expensive. To reduce this we propose an improvement of existing optimization approaches based on user-centered design, focusing on readability, comprehensibility, and user satisfaction as optimization goals. The changes comprise (1) a separate optimization of user interface and representation, (2) a fully automated evaluation of the representation, and (3) qualitative user studies for simultaneously creating and evaluating interface variants. On the basis of these results we are able to find a local optimum of an information visualization in an efficient way.

==> src/expert_interviews.tex <==
\section{\uppercase{Iterative Qualitative User Studies}}
\label{sec:expertinterviews}

% 
% General challenges
% 

\todo[inline]{Wording (variation point, implementation) differs from readability section, maybe adapt it}
\todo[inline]{paragraph is redundant, already mentioned in introduction/approach since it is the basic idea of the paper}


User studies are an established approach to evaluate information visualization. 




User studies etablierter weg
Quantitativ Ansatz aber nicht zielfuhrend
Ansätze mit qualitativem feedback als Alternative 
Besonders für Interaktion, nicht nur simple Wahrnehmung, mit komplexen Aufgaben
Interaktionstechniken als optimierungsziel im Zusammenspiel mit dem UI
Nebenbed‎ingung Integration in gesamt UI, bzw ein Aspekt der itec
Definition itec
Mehrere Varianten des UI
Qualitatives feedback aus xxx
Liefert Vorschläge für neue varianten
Liefert Aussagen zu besserer Variante 
Simple Häufigkeiten 
Messwerte für Trends 



        
%Every visualization has a lot of variation points in representation and interaction with many possible implementations.
%Some of these have substitute functionality and other have complementary functionality.
%All this variations together leads to a huge amount of variants of the  visualization itself and each may have another influence on user performance.
%However, evaluating all variants or at least every implementation of the variation points in a quantitative evaluation is nearly impossible, because of the effort.
%Also not all variation points and implementations are identified at the beginning of the optimization progress, neither all the possible variants as combination of different variation point implementation.
%Furthermore every implementation of a variation point may have variations of its own as well as bugs and weaknesses.
%
%% 
%% First iteration
%% 
%
%A suitable approach to overcome these challenges is the conduction of user studies as a qualitative evaluation.
%Hence multiple variants can be evaluated with less effort.
%Nevertheless it is still impossible to take all variants into account.
%To get an initial set of promising variants we will have a second look at the list of identified aesthetics.
%Since they disclose the variation points in which glyphs differ from each other two undesired effects are observable:
%On the one hand, glyphs are not distinguishable although they are meant to be.
%In this case it is necessary to emphasize their differences, e.g., by using a more prominent visual channel.
%Fox example for recursive disk visualization no differences between methods segments were spotted during the repertory grid interviews although this was intended \cite{Baum2015, Muller2014}.
%
%% 
%% Further iterations
%% 
%
%The results are not only variation point implementations that are superior to other ones, but also bug identification and hints for further improvements.
%These suggestions are used to create new visualization variants.
%Therefore this optimization step should be arranged in an iterative cycle of conducting the user studies and using the feedback to optimize the variants of the visualization.
%Each iteration is one step to a nearly ideal visualization for the specific tasks.
%While these iterative qualitative evaluation some implementations of a variation points may be identified, which seem equal in the given feedback of the users.
%In this case a quantitative evaluation as a controlled experiment may clear the question which one allows a better performance.
%Another way is the use of a configuration option to let the users choose their favored one.
%
%The user studies should be designed within subject, so more than one variant is evaluated in one run.
%The advantage is, that a the subject can compare the different variants for more detailed feedback and can easier produce new ideas, improvements and hints for the varied implementations and the visualization as a whole.
%A tutorial should introduce every part of the visualization and every possible interaction in every tested variant.
%Because not all possible variants can be evaluation within user studies neither, a suitable preselection should be made.
%Therefore clustering the variation points and evaluating one cluster is a possible approach.
%
%The qualitative evaluation instead should be designed as between subject, because of lesser threads to validity caused by the dependencies between the single variants.
%Another advantage of this design is the lesser amount of knowledge the subject must have about the visualization functions similarly to the smaller tutorial that is needed to introduce these functions.

